Evaluation of Programming Models and Performance for Stencil Computation on Current GPU Architectures

Accelerated computing is widely used in high-performance computing. Therefore, it is crucial to experiment and discover how to better utilize GPUGPUs latest generations on relevant applications. In this paper, we present results and share insights about highly tuned stencil-based kernels for NVIDIA Ampere (A100) and Hopper (GH200) architectures. Performance results yield useful insights into the behavior of this type of algorithms for these new accelerators. This knowledge can be leveraged by many scientific applications which involve stencils computations. Further, evaluation of three different programming models: CUDA, OpenACC, and OpenMP target offloading is conducted on aforementioned accelerators. We extensively study the performance and portability of various kernels under each programming model and provide corresponding optimization recommendations. Furthermore, we compare the performance of different programming models on the mentioned architectures. Up to 58% performance improvement was achieved against the previous GPGPU's architecture generation for an highly optimized kernel of the same class, and up to 42% for all classes. In terms of programming models, and keeping portability in mind, optimized OpenACC implementation outperforms OpenMP implementation by 33%. If portability is not a factor, our best tuned CUDA implementation outperforms the optimized OpenACC one by 2.1x.

==> content/tikz_figs/h100-cuda-roofline.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson}{RGB}{220,20,60}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkslateblue}{RGB}{72,61,139}
\definecolor{dodgerblue}{RGB}{30,144,255}
\definecolor{gold}{RGB}{255,215,0}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{limegreen}{RGB}{50,205,50}
\definecolor{mediumpurple}{RGB}{147,112,219}
\definecolor{mediumseagreen}{RGB}{60,179,113}
\definecolor{orange}{RGB}{255,165,0}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(1,0)},
  anchor=south east,
  draw=lightgray204
},
log basis x={10},
log basis y={10},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Arithmetic Intensity [FLOPs/Byte]},
xmajorgrids,
xmin=0.1, xmax=100,
xmode=log,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Performance [GFLOP/sec]},
ymajorgrids,
ymin=100, ymax=200000,
ymode=log,
ytick style={color=black}
]
\addplot [thick, black, forget plot]
table {%
0.497702356433211 32768
0.533669923120631 32768
0.572236765935022 32768
0.613590727341317 32768
0.657933224657568 32768
0.705480231071864 32768
0.756463327554629 32768
0.811130830789687 32768
0.869749002617783 32768
0.93260334688322 32768
1 32768
1.07226722201032 32768
1.14975699539774 32768
1.23284673944207 32768
1.32194114846603 32768
1.41747416292681 32768
1.51991108295293 32768
1.62975083462064 32768
1.74752840000768 32768
1.87381742286038 32768
2.00923300256505 32768
2.15443469003188 32768
2.31012970008316 32768
2.47707635599171 32768
2.65608778294669 32768
2.8480358684358 32768
3.05385550883342 32768
3.27454916287773 32768
3.51119173421513 32768
3.76493580679247 32768
4.03701725859656 32768
4.32876128108306 32768
4.64158883361278 32768
4.97702356433211 32768
5.33669923120631 32768
5.72236765935022 32768
6.13590727341317 32768
6.57933224657568 32768
7.05480231071865 32768
7.56463327554629 32768
8.11130830789687 32768
8.69749002617784 32768
9.3260334688322 32768
10 32768
10.7226722201032 32768
11.4975699539774 32768
12.3284673944207 32768
13.2194114846603 32768
14.174741629268 32768
15.1991108295293 32768
16.2975083462065 32768
17.4752840000768 32768
18.7381742286038 32768
20.0923300256505 32768
21.5443469003188 32768
23.1012970008316 32768
24.7707635599171 32768
26.5608778294669 32768
28.480358684358 32768
30.5385550883342 32768
32.7454916287773 32768
35.1119173421513 32768
37.6493580679247 32768
40.3701725859655 32768
43.2876128108306 32768
46.4158883361278 32768
49.7702356433211 32768
53.3669923120631 32768
57.2236765935022 32768
61.3590727341318 32768
65.7933224657568 32768
70.5480231071865 32768
75.6463327554629 32768
81.1130830789687 32768
86.9749002617783 32768
93.260334688322 32768
100 32768
};
\addplot [thick, black, forget plot]
table {%
0.1 6391.1726
0.107226722201032 6853.04488919049
0.114975699539774 7348.29540564433
0.123284673944207 7879.33630112147
0.132194114846603 8448.75404688862
0.141747416292681 9059.32203130573
0.151991108295293 9714.01406780512
0.162975083462064 10416.0188790546
0.174752840000768 11168.7556278509
0.187381742286038 11975.8905703879
0.200923300256505 12841.3549130095
0.215443469003188 13769.3639594213
0.231012970008316 14764.4376416177
0.247707635599171 15831.4225345221
0.265608778294669 16975.5154615636
0.28480358684358 18202.2888061641
0.305385550883342 19517.7176524152
0.327454916287773 20928.2088871371
0.351119173421513 22440.6324050622
0.376493580679247 24062.3545691309
0.403701725859655 25801.2740888694
0.432876128108306 27665.8604915989
0.464158883361278 29665.195373852
0.497702356433211 31809.0166339137
};
\addplot [thick, black, forget plot]
table {%
0.1 840.886
0.107226722201032 901.654495247373
0.114975699539774 966.81456083202
0.123284673944207 1036.68356334248
0.132194114846603 1111.60180456901
0.141747416292681 1191.93417896687
0.151991108295293 1278.07195089996
0.162975083462064 1370.43466032082
0.174752840000768 1469.47216616886
0.187381742286038 1575.66683743938
0.200923300256505 1689.53590259491
0.215443469003188 1811.63396876215
0.231012970008316 1942.55572298413
0.247707635599171 2082.93882868445
0.265608778294669 2233.46703145091
0.28480358684358 2394.87348926551
0.305385550883342 2567.9443434009
0.327454916287773 2753.5225473756
0.351119173421513 2952.51197261722
0.376493580679247 3165.88181083049
0.403701725859655 3394.67129451222
0.432876128108306 3639.99475860481
0.464158883361278 3903.04706794132
0.497702356433211 4185.10943691697
0.533669923120631 4487.55566973215
0.572236765935022 4811.85885160037
0.613590727341317 5159.59852351131
0.657933224657568 5532.46837549404
0.705480231071864 5932.28449585096
0.756463327554629 6360.99421654102
0.811130830789687 6820.68559779417
0.869749002617783 7313.59759815258
0.93260334688322 7842.13097947243
1 8408.86
1.07226722201032 9016.54495247373
1.14975699539774 9668.1456083202
1.23284673944207 10366.8356334248
1.32194114846603 11116.0180456901
1.41747416292681 11919.3417896687
1.51991108295293 12780.7195089996
1.62975083462064 13704.3466032082
1.74752840000768 14694.7216616886
1.87381742286038 15756.6683743938
2.00923300256505 16895.3590259491
2.15443469003188 18116.3396876215
2.31012970008316 19425.5572298413
2.47707635599171 20829.3882868445
2.65608778294669 22334.6703145091
2.8480358684358 23948.7348926551
3.05385550883342 25679.443434009
3.27454916287773 27535.225473756
3.51119173421513 29525.1197261722
3.76493580679247 31658.8181083049
};
\addplot [thick, black, forget plot]
table {%
0.1 203.9021
0.107226722201032 218.637538329071
0.114975699539774 234.437865851289
0.123284673944207 251.38003915039
0.132194114846603 269.546576248635
0.141747416292681 289.025958516518
0.151991108295293 309.913061627377
0.162975083462064 332.309617655902
0.174752840000768 356.324710571207
0.187381742286038 382.07530753782
0.200923300256505 409.686828612318
0.215443469003188 439.29375761035
0.231012970008316 471.040297119326
0.247707635599171 505.081070847057
0.265608778294669 541.581876727174
0.28480358684358 580.720494449384
0.305385550883342 622.687551347702
0.327454916287773 667.687450864011
0.351119173421513 715.939368109107
0.376493580679247 767.678317370179
0.403701725859655 823.156296764081
0.432876128108306 882.643515611526
0.464158883361278 946.429710510196
0.497702356433211 1014.8255565168
0.533669923120631 1088.16418031135
0.572236765935022 1166.80278271359
0.613590727341317 1251.12437845422
0.657933224657568 1341.5396616745
0.705480231071864 1438.48900624038
0.756463327554629 1542.44461061377
0.811130830789687 1653.91279772762
0.869749002617783 1773.43648106672
0.93260334688322 1901.59780896517
1 2039.021
1.07226722201032 2186.37538329071
1.14975699539774 2344.37865851289
1.23284673944207 2513.8003915039
1.32194114846603 2695.46576248635
1.41747416292681 2890.25958516518
1.51991108295293 3099.13061627377
1.62975083462064 3323.09617655902
1.74752840000768 3563.24710571207
1.87381742286038 3820.7530753782
2.00923300256505 4096.86828612318
2.15443469003188 4392.9375761035
2.31012970008316 4710.40297119327
2.47707635599171 5050.81070847058
2.65608778294669 5415.81876727174
2.8480358684358 5807.20494449384
3.05385550883342 6226.87551347702
3.27454916287773 6676.87450864011
3.51119173421513 7159.39368109107
3.76493580679247 7676.78317370178
4.03701725859656 8231.56296764081
4.32876128108306 8826.43515611526
4.64158883361278 9464.29710510196
4.97702356433211 10148.255565168
5.33669923120631 10881.6418031135
5.72236765935022 11668.0278271359
6.13590727341317 12511.2437845422
6.57933224657568 13415.396616745
7.05480231071865 14384.8900624038
7.56463327554629 15424.4461061377
8.11130830789687 16539.1279772762
8.69749002617784 17734.3648106672
9.3260334688322 19015.9780896517
10 20390.21
10.7226722201032 21863.7538329071
11.4975699539774 23443.7865851289
12.3284673944207 25138.003915039
13.2194114846603 26954.6576248635
14.174741629268 28902.5958516518
15.1991108295293 30991.3061627377
};
\addplot [semithick, orange, opacity=0.6, mark=*, mark size=3, mark options={solid}, only marks]
table {%
0.964180044686989 2266.4486151025
};
\addlegendentry{gmem}
\addplot [semithick, gold, opacity=0.6, mark=*, mark size=3, mark options={solid}, only marks]
table {%
1.15352963509133 2309.55287324653
};
\addlegendentry{gmem-opt}
\addplot [semithick, dodgerblue, opacity=0.6, mark=*, mark size=3, mark options={solid}, only marks]
table {%
1.23447674346749 2146.45111934887
};
\addlegendentry{smem}
\addplot [semithick, darkslateblue, opacity=0.6, mark=*, mark size=3, mark options={solid}, only marks]
table {%
1.41657862882755 2095.52244181762
};
\addlegendentry{smem-opt}
\addplot [semithick, limegreen, opacity=0.6, mark=*, mark size=3, mark options={solid}, only marks]
table {%
1.30917583375995 1390.77881620284
};
\addlegendentry{st\_reg}
\addplot [semithick, mediumseagreen, opacity=0.6, mark=*, mark size=3, mark options={solid}, only marks]
table {%
1.33094472193052 1405.43584074976
};
\addlegendentry{st\_reg-opt}
\addplot [semithick, crimson, opacity=0.6, mark=*, mark size=3, mark options={solid}, only marks]
table {%
1.67384450670377 1398.17291192229
};
\addlegendentry{st\_semi}
\addplot [semithick, mediumpurple, opacity=0.6, mark=*, mark size=3, mark options={solid}, only marks]
table {%
1.68936117010478 1415.93076425078
};
\addlegendentry{st\_semi-opt}
\draw (axis cs:93.260334688322,32768) node[
  scale=0.9,
  anchor=south east,
  text=black,
  rotate=0.0
]{DP-H100: 32.0 TFLOP/s};
\draw (axis cs:0.114975699539774,8179.26648978111) node[
  scale=0.9,
  anchor=south west,
  text=black,
  rotate=42.3
]{L1-H100: 63911.7 GB/s};
\draw (axis cs:0.114975699539774,1076.14535109349) node[
  scale=0.9,
  anchor=south west,
  text=black,
  rotate=42.3
]{L2-H100: 8408.9 GB/s};
\draw (axis cs:0.114975699539774,260.94892410291) node[
  scale=0.9,
  anchor=south west,
  text=black,
  rotate=42.3
]{HBM-H100: 2039.0 GB/s};
\end{axis}

\end{tikzpicture}

